Classifying the Dynamics of Architected Materials by Groupoid Methods

We consider synthetic materials consisting of self-coupled identical resonators carrying classical internal degrees of freedom. The architecture of such material is specified by the positions and orientations of the resonators. Our goal is to calculate the smallest C*-algebra that covers the dynamical matrices associated to a fixed architecture and adjustable internal structures. We give the answer in terms of a groupoid C*-algebra that can be canonically associated to a uniformly discrete subset of the group of isometries of the Euclidean space. Our result implies that the isomorphism classes of these C*-algebras split these architected materials into classes containing materials that are identical from the dynamical point of view.

==> notation.tex <==
% -- Particular notation for this paper -------------------------------

\DeclareMathOperator{\Iso}{\mathrm{Iso}}

\newcommand{\Grp}{\mathbf{Grp}}
\newcommand{\AlgC}{\mathbf{Alg}_{\mathbb{C}}}
\newcommand{\CAlg}{\mathbf{C^\ast Alg}}
\DeclareMathOperator{\Obj}{\mathrm{Obj}}
\DeclareMathOperator{\Hom}{\mathrm{Hom}}
\DeclareMathOperator{\im}{\mathrm{im}}
%\DeclareMathOperator{\ker}{\mathrm{ker}}

% -- Math headings ----------------------------------------------------

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{fancyproclaim}
%\newtheorem*{vartheorem}{ }
%\theoremstyle{statement}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{exercise}[theorem]{Exercise}
%\theoremstyle{fancystatement}
%\newtheorem*{varremark}{ }

\numberwithin{equation}{section}
\numberwithin{figure}{section}
%\renewcommand{\theenumi}{\roman{enumi}}


% -- BB symbols -------------------------------------------------------

\newcommand{\BM}{{\mathbb B}}
\newcommand{\CM}{{\mathbb C}}
\newcommand{\NM}{{\mathbb N}}
\newcommand{\PM}{{\mathbb P}}
\newcommand{\QM}{{\mathbb Q}}
\newcommand{\RM}{{\mathbb R}}
\newcommand{\SM}{{\mathbb S}}
\newcommand{\TM}{{\mathbb T}}
\newcommand{\ZM}{{\mathbb Z}}
%\newcommand{\PM}{{\mathbb P}}
\newcommand{\LM}{{\mathbb L}}
\newcommand{\KM}{{\mathbb K}}
\newcommand{\HM}{{\mathbb H}}
\newcommand{\DM}{{\mathbb D}}
\newcommand{\EM}{{\mathbb E}}
\newcommand{\GM}{{\mathbb G}}
\newcommand{\UM}{{\mathbb U}}
\newcommand{\WM}{{\mathbb W}}
\newcommand{\FM}{{\mathbb F}}
\newcommand{\imathM}{{\mathbb I}}

% -- Bold symbols -----------------------------------------------------

\newcommand{\PP}{{\bf P}}
\newcommand{\QQ}{{\bf Q}}
\newcommand{\HH}{{\bf H}}
\newcommand{\UU}{{\bf U}}
\newcommand{\pp}{{\bf p}}
\newcommand{\BB}{{\bf B}}
\newcommand{\EE}{{\bf E}}

% -- Cal symbols ------------------------------------------------------

\newcommand{\Aa}{{\mathcal A}}
\newcommand{\Ee}{{\mathcal E}}
\newcommand{\Ii}{{\mathcal I}}
\newcommand{\Pp}{{\mathcal P}}
\newcommand{\Bb}{{\mathcal B}}
\newcommand{\Dd}{{\mathcal D}}
\newcommand{\Ff}{{\mathcal F}}
\newcommand{\Gg}{{\mathcal G}}
\newcommand{\Ww}{{\mathcal W}}
\newcommand{\Uu}{{\mathcal U}}
\newcommand{\Vv}{{\mathcal V}}
\newcommand{\Ss}{{\mathcal S}}
\newcommand{\Oo}{{\mathcal O}}
\newcommand{\Tt}{{\mathcal T}}
\newcommand{\Rr}{{\mathcal R}}
\newcommand{\Nn}{{\mathcal N}}
\newcommand{\Mm}{{\mathcal M}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Yy}{{\mathcal Y}}
\newcommand{\Jj}{{\mathcal J}}
\newcommand{\imathi}{{\mathcal I}}
\newcommand{\Ll}{{\mathcal L}}
\newcommand{\Qq}{{\mathcal Q}}
\newcommand{\Kk}{{\mathcal K}}
\newcommand{\Hh}{{\mathcal H}}
\newcommand{\Xx}{{\mathcal X}}

% -- Special notation -------------------------------------------------

\newcommand{\cor}{{\mbox{\rm\tiny cor}}}
\newcommand{\av}{{\mbox{\rm\tiny av}}}
\def\essinf{\mathop{\rm ess\,inf}}
\def\esssup{\mathop{\rm ess\,sup}}
\newcommand{\Zh}{{\widehat{Z}}}
\newcommand{\one}{{\bf 1}}
\newcommand{\nul}{{\bf 0}}
\newcommand{\inv}{{\mbox{\rm\tiny inv}}}
\newcommand{\up}{{\mbox{\rm\tiny upp}}}
\newcommand{\TR}{{\rm Tr}} 
%\newcommand{\tr}{{\rm tr}} 
\newcommand{\ev}{{\mbox{\rm ev}}}


\newcommand{\SF}{{\rm Sf}} 
\newcommand{\Ch}{{\rm Ch}} 
\newcommand{\imathnd}{{\rm Ind}} 
\newcommand{\Ker}{{\rm Ker}} 
\newcommand{\Ran}{{\rm Ran}} 
\newcommand{\sgn}{{\rm sgn}} 
\newcommand{\sign}{{\rm sign}} 
\newcommand{\Sig}{{\rm Sig}} 
\newcommand{\Exp}{{\rm Exp}} 
\newcommand{\PI}{{\rm \Pi}} 
\newcommand{\Ti}{\varphi}

%\newcommand{\diag}{{\mbox{\rm diag}}}
\newcommand{\redu}{{\mbox{\rm\tiny red}}}
\newcommand{\ph}{{\mbox{\rm\tiny ph}}}
\newcommand{\ess}{{\mbox{\rm\tiny ess}}}
\newcommand{\sym}{{\mbox{\rm\tiny sym}}}
\newcommand{\Wind}{{\mbox{\rm Wind}}}
\newcommand{\GFunc}{f_{\mbox{\rm\tiny Ind}}}
\newcommand{\FFunc}{f_{\mbox{\rm\tiny Exp}}}
\newcommand{\tFFunc}{\tilde{f}_{\mbox{\rm\tiny Exp}}}


\newcommand{\frakc}{{\mathfrak c}}
\newcommand{\frakd}{{\mathfrak d}}

\newcommand{\Rstruc}{{\tau}}
\newcommand{\AaR}{{\mathcal A}^\Re}
\newcommand{\AaI}{{\mathcal A}^\imathm}

\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[2]{\langle #1|#2\rangle}        %BRA & KET
\newcommand{\ketbra}[2]{|#1\rangle\langle#2|}
\newcommand{\nk}{\kappa}
%\newcommand{\proof}{{\noindent {\it Proof.} \hspace{0.05cm}}}
%\newcommand{\qed}{$\square$}
\newcommand{\I}{{\rm i}}

\newcommand{\id}{\mathrm{id}}


